PI(D) tuning for Flight Control Systems via Incremental Nonlinear Dynamic Inversion

Previous results reported in the robotics literature show the relationship between time-delay control (TDC) and proportional-integral-derivative control (PID). In this paper, we show that incremental nonlinear dynamic inversion (INDI) - more familiar in the aerospace community - are in fact equivalent to TDC. This leads to a meaningful and systematic method for PI(D)-control tuning of robust nonlinear flight control systems via INDI. We considered a reformulation of the plant dynamics inversion which removes effector blending models from the resulting control law, resulting in robust model-free control laws like PI(D)-control.

==> figures/this_rates_v5b.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.850,0.325,0.098}\fontsize{11}{11}\selectfont\strut}%
\psfrag{037}[tc][tc]{\matlabtextA $\delta$ (deg)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{039}[tc][tc]{\matlabtextB time~(s)}%
\psfrag{042}[tc][tc]{\matlabtextB time~(s)}%
\psfrag{043}[bc][bc]{\matlabtextB $q$ (deg/s)}%
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.447,0.741}\fontsize{11}{11}\selectfont\strut}%
\psfrag{040}[bc][bc]{\matlabtextC $\alpha$ (deg)}%
%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{11}{11}\bfseries\boldmath\selectfont\strut}%
\psfrag{036}[bc][bc]{\matlabtextD }%
\psfrag{038}[bc][bc]{\matlabtextD }%
\psfrag{041}[bc][bc]{\matlabtextD }%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextE{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextE $0$}%
\psfrag{001}[ct][ct]{\matlabtextE $5$}%
\psfrag{002}[ct][ct]{\matlabtextE $10$}%
\psfrag{003}[ct][ct]{\matlabtextE $15$}%
\psfrag{004}[ct][ct]{\matlabtextE $20$}%
\psfrag{012}[ct][ct]{\matlabtextE $0$}%
\psfrag{013}[ct][ct]{\matlabtextE $5$}%
\psfrag{014}[ct][ct]{\matlabtextE $10$}%
\psfrag{015}[ct][ct]{\matlabtextE $15$}%
\psfrag{016}[ct][ct]{\matlabtextE $20$}%
\psfrag{024}[ct][ct]{\matlabtextE $0$}%
\psfrag{025}[ct][ct]{\matlabtextE $5$}%
\psfrag{026}[ct][ct]{\matlabtextE $10$}%
\psfrag{027}[ct][ct]{\matlabtextE $15$}%
\psfrag{028}[ct][ct]{\matlabtextE $20$}%
%
%% </xtick>
%
%% <ytick>
%
\providecommand\matlabtextF{\color[rgb]{0.850,0.325,0.098}\fontsize{10}{10}\selectfont\strut}%
\psfrag{005}[lc][lc]{\matlabtextF $-6$}%
\psfrag{006}[lc][lc]{\matlabtextF $-4$}%
\psfrag{007}[lc][lc]{\matlabtextF $-2$}%
\psfrag{008}[lc][lc]{\matlabtextF $0$}%
\psfrag{009}[lc][lc]{\matlabtextF $2$}%
\psfrag{010}[lc][lc]{\matlabtextF $4$}%
\psfrag{011}[lc][lc]{\matlabtextF $6$}%
%
\providecommand\matlabtextG{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{029}[rc][rc]{\matlabtextG $-6$}%
\psfrag{030}[rc][rc]{\matlabtextG $-4$}%
\psfrag{031}[rc][rc]{\matlabtextG $-2$}%
\psfrag{032}[rc][rc]{\matlabtextG $0$}%
\psfrag{033}[rc][rc]{\matlabtextG $2$}%
\psfrag{034}[rc][rc]{\matlabtextG $4$}%
\psfrag{035}[rc][rc]{\matlabtextG $6$}%
%
\providecommand\matlabtextH{\color[rgb]{0.000,0.447,0.741}\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[rc][rc]{\matlabtextH $-6$}%
\psfrag{018}[rc][rc]{\matlabtextH $-4$}%
\psfrag{019}[rc][rc]{\matlabtextH $-2$}%
\psfrag{020}[rc][rc]{\matlabtextH $0$}%
\psfrag{021}[rc][rc]{\matlabtextH $2$}%
\psfrag{022}[rc][rc]{\matlabtextH $4$}%
\psfrag{023}[rc][rc]{\matlabtextH $6$}%
%
%% </ytick>

==> referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}

%
\begin{thebibliography}{99.}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% My euroGNC bib
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Conference article
\bibitem{Acquatella-e} Paul Acquatella B., Wouter Falkena, Erik-Jan van Kampen, and Qi Ping Chu. (2012).
Robust nonlinear spacecraft attitude control using incremental nonlinear dynamic inversion. 
In \textit{AIAA Guidance, Navigation and Control Conference}, American Institute of Aeronautics and Astronautics, Inc. (AIAA-2012-4623).
% Journal article
\bibitem{Adams-e} Richard J. Adams and Siva S. Banda. (1993).
Robust flight control design using dynamic inversion and structures singular value synthesis. 
\textit{IEEE Transactions on Control Systems Technology}, Vol. 1, No. 2, pp. 80-92, 
doi: 10.1109/87.238401
% Conference article
\bibitem{Balas-e} Gary J. Balas, William L. Garrard, and Jakob Reiner. (1992).
Robust dynamic inversion control laws for aircraft control. 
In \textit{AIAA Guidance, Navigation and Control Conference}, American Institute of Aeronautics and Astronautics, Inc. (AIAA-92-4329).
% Journal article
\bibitem{Bacon1-e} Barton J. Bacon and Aaron J. Ostroff. (2000). 
Reconfigurable flight control using nonlinear dynamic inversion with a special accelerometer implementation.
In \textit{AIAA Guidance, Navigation, and Control Conference and Exhibit}. American Institute of Aeronautics and Astronautics, Inc. (AIAA-2000-4565).
\bibitem{Bacon2-e} Barton J. Bacon, Aaron J. Ostroff, and Suresh M. Joshi. (2000). 
Nonlinear dynamic inversion reconfigurable controller utilizing a fault-tolerant accelerometer approach.
In \textit{DASC 19th Digital Avionics Systems Conference}, Vol. 2, pp.6F5/1-6F5/8,
doi: 10.1109/DASC.2000.884920
\bibitem{Bacon3-e} Barton J. Bacon, Aaron J. Ostroff, and Suresh M. Joshi. (2001).
Reconfigurable NDI controller using inertial sensor failure detection \& isolation.
\textit{IEEE Transactions on Aerospace and Electronic Systems}. Vol. 37, No. 4, pp. 1373-1383,
doi: 10.1109/7.976972
% Journal article
\bibitem{Bugajski-e} Daniel J. Bugajski and Dale F. Enns. (1992). 
Nonlinear control law with application to high angle-of-attack flight.
\textit{Journal of Guidance, Control, and Dynamics}, Vol. 15, No. 3, pp. 761-767, 
doi: 10.2514/3.20902
% Conference article
\bibitem{Campbell-e} Stefan F. Campbell and John T. Kaneshige. (2010).
A nonlinear dynamic inversion L1 adaptive controller for a Generic Transport Model.
In \textit{American Control Conference (ACC), 2010}, pp. 862-867.
% Journal article
\bibitem{Chen-e} H. B. Chen and S. G. Zhang. (2008). 
Robust dynamic inversion flight control law design.
In \textit{ISSCAA 2nd International Symposium on Systems and Control in Aerospace and Astronautics}, 
doi: 10.1109/ISSCAA.2008.4776382
% Lecture notes
\bibitem{Chu1-e} Q. P. Chu. (2010a).
\textit{Advanced Flight Control}. Lecture notes, Delft University of Technology, Faculty of Aerospace Engineering.
\bibitem{Chu2-e} Q. P. Chu. (2010b).
\textit{Spacecraft Attitude Control Systems}. Lecture notes, Delft University of Technology, Faculty of Aerospace Engineering.  
% Journal article
\bibitem{Enns1-e} D. F. Enns., D. J. Bugajski, R. C. Hendrick, and G. Stein. (1994).
Dynamic inversion: an evolving methodology for flight control. 
\textit{International Journal of Control}, Vol. 59, No. 1, pp. 71-91, 
doi: 10.1080/00207179408923070
% Conference article
\bibitem{Enns2-e} D. F. Enns. (1990).
Robustness of dynamic inversion vs. mu-synthesis: lateral-directional flight control example. 
In \textit{AIAA Guidance, Navigation and Control Conference}, American Institute of Aeronautics and Astronautics, Inc. (AIAA-90-3338).
% Conference article
\bibitem{Goman-e} M. G. Goman and E. N. Kolesnikov. (1998).
Robust nonlinear dynamic inversion method for an aircraft motion control. 
In \textit{AIAA Guidance, Navigation and Control Conference}, American Institute of Aeronautics and Astronautics, Inc. (AIAA-98-4208).
% Journal article
\bibitem{Kim-e} S. H. Kim, Y. S. Kim, and C. Song. (2004).
A robust adaptive nonlinear control approach to missile autopilot design. 
\textit{Control Engineering Practice}, Vol. 33, No. 6, pp. 1732-1742, 
doi: 10.2514/1.49978
% Monograph
\bibitem{Khalil-e} Hassan K. Khalil. (2002). 
\textit{Nonlinear systems} (3rd ed.).
Prentice Hall.
% Monograph
\bibitem{Krstic-e} Miroslav Krsti\'c, Ioannis Kanellakopoulos, and Petar Kokotovi\'c. (1995). 
\textit{Nonlinear and adaptive control design}.
John Wiley \& Sons.
% Conference article
\bibitem{Lombaerts-e} T.J.J. Lombaerts, H.O. Huisman, Q. P. Chu, J. A. Mulder, and D. A. Joosten. (2008).
Flight control reconfiguration based on online physical model identification and nonlinear dynamic inversion.
In \textit{AIAA Guidance, Navigation and Control Conference}, American Institute of Aeronautics and Astronautics, Inc. (AIAA-2008-7435).
% Conference article
\bibitem{Schumacher-e} Corey Schumacher. (1999).
Adaptive flight control using dynamic inversion and neural networks.
In \textit{AIAA Guidance, Navigation and Control Conference}, American Institute of Aeronautics and Astronautics, Inc. (AIAA-99-4086).
% Journal article
\bibitem{Sieberling-e} S. Sieberling, Q. P. Chu, and J. A. Mulder. (2010).
Robust flight control using incremental nonlinear dynamic inversion and angular acceleration prediction. 
\textit{Journal of Guidance, Control, and Dynamics}, Vol. 33, No. 6, pp. 1732-1742, 
doi: 10.2514/1.49978 
% Conference article
\bibitem{Smith0-e} P. R. Smith. (1994).
Functional control law design using exact nonlinear dynamic inversion. 
In \textit{AIAA Atmospheric Flight Mechanics Conference}, American Institute of Aeronautics and Astronautics, Inc. (AIAA-94-3516).
% Conference article
\bibitem{Smith1-e} P. R. Smith. (1995).
Translational motion control of VSTOL aircraft using nonlinear dynamic inversion.
In \textit{AIAA Atmospheric Flight Mechanics Conference}, American Institute of Aeronautics and Astronautics, Inc. (AIAA-95-3452).
% Conference article
\bibitem{Smith2-e} P. R. Smith. (1998).
A simplified approach to nonlinear dynamic inversion based flight control. 
In \textit{AIAA Atmospheric Flight Mechanics Conference}, American Institute of Aeronautics and Astronautics, Inc. (AIAA-98-4461).
% Conference article
\bibitem{Smith3-e} P. R. Smith and A. Berry. (2000).
Flight test experience of a nonlinear dynamic inversion control law on the VAAC Harrier. 
In \textit{AIAA Atmospheric Flight Mechanics Conference}, American Institute of Aeronautics and Astronautics, Inc. (AIAA-2000-3914).
% Monograph
\bibitem{Snell2-e} S. A. Snell. (1991). \textit{Nonlinear dynamic-inversion flight control of supermaneuvrable aircraft}.
PhD thesis, University of Minnesota, Aerospace Engineering and Mechanics Department. 
%
% Monograph
\bibitem{Sonneveldt-e} Lars Sonneveldt. (2010). \textit{Adaptive backstepping flight control for modern fighter aircraft}.
PhD thesis, Delft University of Technology, Faculty of Aerospace Engineering. 
% Conference article
\bibitem{Weerdt-e} E. de Weerdt, E. van Kampen, D. van Gemert, Q. P. Chu, and J. A. Mulder. (2008).
Adaptive nonlinear dynamic inversion for spacecraft attitude control with fuel sloshing.
In \textit{AIAA Guidance, Navigation and Control Conference}, American Institute of Aeronautics and Astronautics, Inc. (AIAA-2008-7162).
\end{thebibliography}

